X-ray flares of the young planet host DS Tuc A

Abridged. We observed the 40 Myr old star DS Tuc A with XMM-Newton and recorded two X-ray bright flares, with the second event occurring about 12 ks after the first one. Their duration from the rise to the end of the decay was of about 8-10 ks in soft X-rays (0.3-10 keV). The flares were also recorded in the band 200-300 nm with the UVM2 filter of the Optical Monitor. The duration of the flares in UV was about 3 ks. The observed delay between the peak in the UV band and in X-rays is a probe of the heating phase followed by the evaporation and increase of density and emission measure of the flaring loop. The coronal plasma temperature at the two flare peaks reached 54-55 MK. The diagnostics based on temperatures and time scales of the flares applied to these two events allow us to infer a loop length of 5-7 x 10^10 cm, which is about the size of the stellar radius. We also infer values of electron density at the flare peaks of 2.3-6.5 x 10^11 cm^-3 , and a minimum magnetic field strength of order of 300-500 G needed to confine the plasma. The energy released during the flares was of order of 5-8 x 10^34 erg in the band 0.3-10 keV and 0.9-2.7 x 10^33 erg in the UV band (200-300 nm). We speculate that the flares were associated with Coronal Mass Ejections (CMEs) that hit the planet about 3.3 hr after the flares and dramatically increasing the rate of evaporation of the planet. From the RGS spectra we retrieved the emission measure distribution and the abundances of coronal metals during the quiescent and the flaring states. In agreement with what inferred from time resolved spectroscopy and EPIC spectra, also from the analysis of RGS spectra during the flares we infer a high electron density.

==> RGSfluxtextable_old.tex <==

\begin{table*}
\caption{Measured fluxes of emission lines and continuum intervals in the X-ray spectrum of DS~Tuc.}
\label{tab:RGSfluxes}
\begin{center}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{r@{$\div$}llcr@{$\;\pm\;$}lr@{$\;\pm\;$}lc}
\hline\hline
 \multicolumn{2}{c}{ } & & & \multicolumn{2}{c}{quiescent} & \multicolumn{2}{c}{flaring} & \\
\multicolumn{2}{c}{$\lambda^{a}$} & Ion & $\log T_{\rm max}^{b}$ & \multicolumn{2}{c}{Flux$^{c}$} & \multicolumn{2}{c}{Flux$^{c}$} & EMD$^{d}$ \\
\hline
\multicolumn{ 9}{c}{\it Lines} \\
\hline
\multicolumn{2}{r}{ 8.42\hspace{5mm} } &                                                    {Mg}{XII} {Mg}{XII} &  7.00 &         5.7 &         3.5 &        32.4 &        10.1 & $\ast$ \\
\multicolumn{2}{r}{ 9.17\hspace{5mm} } &                                                               {Mg}{XI} &  6.80 &        20.0 &         3.9 &        32.0 &         9.1 & $\ast$ \\
\multicolumn{2}{r}{ 9.23\hspace{5mm} } &                                                               {Mg}{XI} &  6.80 &         3.2 &         3.2 &        27.1 &         8.8 & \\
\multicolumn{2}{r}{ 9.31\hspace{5mm} } &                                                               {Mg}{XI} &  6.80 &        14.2 &         3.4 &         7.7 &         7.8 & \\
\multicolumn{2}{r}{10.62\hspace{5mm} } &                   {Fe}{XIX} {Fe}{XIX} {Fe}{XVII} {Fe}{XXIV} {Fe}{XXIV} &  7.30 &         1.6 &         2.6 &        51.9 &        12.8 & $\ast$ \\
\multicolumn{2}{r}{10.98\hspace{5mm} } &         {Fe}{XXIII} {Ne}{IX} {Na}{X} {Fe}{XXIII} {Fe}{XVII} {Fe}{XXIV} &  7.20 &        22.8 &         4.5 &        62.1 &        13.8 & $\ast$ \\
\multicolumn{2}{r}{11.43\hspace{5mm} } &                                      {Fe}{XXII} {Fe}{XXIV} {Fe}{XVIII} &  7.20 &        15.3 &         4.8 &        41.7 &        13.1 & $\ast$ \\
\multicolumn{2}{r}{11.74\hspace{5mm} } &                                                            {Fe}{XXIII} &  7.20 &         0.8 &         2.7 &        27.1 &        12.6 & $\ast$ \\
\multicolumn{2}{r}{11.77\hspace{5mm} } &                                                             {Fe}{XXII} &  7.10 &        13.3 &         4.5 &        20.8 &        12.5 & $\ast$ \\
\multicolumn{2}{r}{12.13\hspace{5mm} } &                                             {Fe}{XVII} {Ne}{X} {Ne}{X} &  6.75 &       106.4 &         8.4 &       201.8 &        18.6 & $\ast$ \\
\multicolumn{2}{r}{12.28\hspace{5mm} } &                                                   {Fe}{XXI} {Fe}{XVII} &  7.05 &        20.9 &         6.0 &        54.0 &        14.8 & $\ast$ \\
\multicolumn{2}{r}{12.83\hspace{5mm} } &                                             {Fe}{XX} {Fe}{XX} {Fe}{XX} &  7.05 &        27.8 &         5.5 &        41.6 &        12.8 & $\ast$ \\
\multicolumn{2}{r}{13.45\hspace{5mm} } &                                 {Fe}{XIX} {Ne}{IX} {Fe}{XIX} {Fe}{XXI} &  6.60 &        57.1 &         7.2 &       127.2 &        15.6 & $\ast$ \\
\multicolumn{2}{r}{13.52\hspace{5mm} } &                                                     {Ne}{IX} {Fe}{XIX} &  6.95 &        30.3 &         6.5 &        34.9 &        13.4 & \\
\multicolumn{2}{r}{13.70\hspace{5mm} } &                                                               {Ne}{IX} &  6.55 &        30.5 &         6.2 &        48.0 &        12.6 & \\
\multicolumn{2}{r}{13.74\hspace{5mm} } &                                                              {Fe}{XIX} &  6.95 &        13.1 &         4.7 &         5.9 &         7.6 & \\
\multicolumn{2}{r}{13.82\hspace{5mm} } &                                                   {Fe}{XIX} {Fe}{XVII} &  6.90 &        12.3 &         4.0 &        35.8 &         9.2 & \\
\multicolumn{2}{r}{14.20\hspace{5mm} } &                                    {Fe}{XVIII} {Fe}{XVIII} {Fe}{XVIII} &  6.90 &        42.4 &         4.8 &        65.0 &         9.7 & $\ast$ \\
\multicolumn{2}{r}{14.37\hspace{5mm} } &                                    {Fe}{XVIII} {Fe}{XVIII} {Fe}{XVIII} &  6.90 &        15.0 &         3.8 &        28.0 &         8.7 & $\ast$ \\
\multicolumn{2}{r}{14.54\hspace{5mm} } &                                    {Fe}{XVIII} {Fe}{XVIII} {Fe}{XVIII} &  6.90 &         5.6 &         3.5 &        23.8 &         8.6 & $\ast$ \\
\multicolumn{2}{r}{15.01\hspace{5mm} } &                                                             {Fe}{XVII} &  6.75 &        97.9 &         5.9 &       152.9 &        11.8 & $\ast$ \\
\multicolumn{2}{r}{15.18\hspace{5mm} } &                                          {Fe}{XIX} {O}{VIII} {O}{VIII} &  6.50 &        19.7 &         4.9 &        42.5 &        10.6 & $\ast$ \\
\multicolumn{2}{r}{15.26\hspace{5mm} } &                                                             {Fe}{XVII} &  6.75 &        26.2 &         4.7 &         8.2 &         8.7 & $\ast$ \\
\multicolumn{2}{r}{16.01\hspace{5mm} } &                                        {Fe}{XVIII} {O}{VIII} {O}{VIII} &  6.50 &        34.1 &         4.5 &       100.0 &        10.4 & $\ast$ \\
\multicolumn{2}{r}{16.07\hspace{5mm} } &                                                            {Fe}{XVIII} &  6.85 &        35.7 &         4.5 &        40.0 &         9.0 & $\ast$ \\
\multicolumn{2}{r}{16.78\hspace{5mm} } &                                                             {Fe}{XVII} &  6.75 &        49.5 &         4.6 &       109.1 &        10.3 & $\ast$ \\
\multicolumn{2}{r}{17.05\hspace{5mm} } &                                                             {Fe}{XVII} &  6.75 &        76.3 &         6.6 &       215.8 &        15.7 & \\
\multicolumn{2}{r}{17.10\hspace{5mm} } &                                                             {Fe}{XVII} &  6.70 &        59.9 &         7.7 &        34.5 &        14.0 & \\
\multicolumn{2}{r}{17.62\hspace{5mm} } &                                                            {Fe}{XVIII} &  6.90 &         7.9 &         3.0 &         8.7 &         6.5 & $\ast$ \\
\multicolumn{2}{r}{18.63\hspace{5mm} } &                                                               {O}{VII} &  6.35 &         9.8 &         3.1 &        17.2 &         7.4 & $\ast$ \\
\multicolumn{2}{r}{18.97\hspace{5mm} } &                                                    {O}{VIII} {O}{VIII} &  6.50 &       213.9 &         8.8 &       516.6 &        18.8 & $\ast$ \\
\multicolumn{2}{r}{21.60\hspace{5mm} } &                                                               {O}{VII} &  6.30 &        46.4 &         7.1 &        74.1 &        14.0 & $\ast$ \\
\multicolumn{2}{r}{21.81\hspace{5mm} } &                                                               {O}{VII} &  6.30 &         0.7 &         3.4 &        14.2 &        11.5 & \\
\multicolumn{2}{r}{22.10\hspace{5mm} } &                                                               {O}{VII} &  6.30 &        37.8 &         6.8 &        28.8 &        11.5 & \\
\multicolumn{2}{r}{24.78\hspace{5mm} } &                                                      {N}{VII} {N}{VII} &  6.30 &        25.4 &         5.3 &        72.1 &        12.0 & $\ast$ \\
\multicolumn{2}{r}{33.73\hspace{5mm} } &                                                        {C}{VI} {C}{VI} &  6.15 &        33.1 &         8.9 &        98.4 &        19.2 & $\ast$ \\
\hline
\multicolumn{ 9}{c}{\it Continuum} \\
\hline
            $[ 8.49 $ & $  8.90]$ &                                                                        &  7.80 &        25.5 &         4.2 &       192.1 &        11.6 & $\ast$ \\
            $[29.70 $ & $ 30.36]$ &                                                                        &  6.45 &        27.9 &        11.4 &       165.3 &        21.3 & $\ast$ \\
\hline
\end{tabular}
}
\end{center}
$^a$~Wavelengths (\AA).
$^b$~Temperature (K) of maximum emissivity.
$^c$~Observed fluxes (${\rm 10^{-6}\,ph\,s^{-1}\,cm^{-2}}$) with uncertainties at the 68\% confidence level.
$^d$~Flux measurements selected for the EMD reconstruction.
\end{table*}



==> modeltextable.tex <==
\begin{table}[t]
\caption{EMD and abundances of DS Tuc.}
% Bottom: first ionization potential (F.I.P.) and abundances relative to the solar ones for the measured ion lines. }
\label{tab:RGSmodel}
\begin{center}
\resizebox{0.79\columnwidth}{!}{
\begin{tabular}{c@{\hspace{3mm}}c@{\hspace{3mm}}c}
\hline\hline
log T (K) & log EMD (cm$^{-3}$) & log EMD (cm$^{-3}$) \\
% log T  & log EMD  & log EMD  \\
%  Units: K & cm$^{-3}$ & cm$^{-3}$ \\
Phase      & quiescent & flaring \\
\hline
6.00 & 48.43$^{+ 1.23}_{- 0.66}$  & 49.09$^{+ 0.73}_{- 1.44}$  \\
6.10 & 48.91$^{+ 0.99}_{- 0.54}$  & 49.63$^{+ 0.72}_{- 0.86}$  \\
6.20 & 50.18$^{+ 0.48}_{- 0.54}$  & 50.28$^{+ 0.47}_{- 0.74}$  \\
6.30 & 50.01$^{+ 0.70}_{- 0.40}$  & 50.81$^{+ 0.46}_{- 0.66}$  \\
6.40 & 51.24$^{+ 0.17}_{- 0.64}$  & 50.42$^{+ 0.76}_{- 0.36}$  \\
6.50 & 51.70$^{+ 0.11}_{- 0.50}$  & 51.64$^{+ 0.54}_{- 0.30}$  \\
6.60 & 51.50$^{+ 0.39}_{- 0.18}$  & 52.55$^{+ 0.10}_{- 0.38}$  \\
6.70 & 52.00$^{+ 0.27}_{- 0.14}$  & 52.28$^{+ 0.28}_{- 0.17}$  \\
6.80 & 52.39$^{+ 0.03}_{- 0.30}$  & 52.01$^{+ 0.49}_{- 0.24}$  \\
6.90 & 51.86$^{+ 0.36}_{- 0.38}$  & 52.18$^{+ 0.36}_{- 0.22}$  \\
7.00 & 52.10$^{+ 0.26}_{- 0.27}$  & 52.53$^{+ 0.13}_{- 0.29}$  \\
7.10 & 52.44$^{+ 0.07}_{- 0.33}$  & 52.49$^{+ 0.32}_{- 0.12}$  \\
7.20 & 51.29$^{+ 0.59}_{- 0.30}$  & 52.70$^{+ 0.21}_{- 0.34}$  \\
7.30 & 50.88$^{+ 0.62}_{- 0.33}$  & 52.19$^{+ 0.51}_{- 0.16}$  \\
7.40 & 50.81$^{+ 0.55}_{- 0.58}$  & 52.57$^{+ 0.44}_{- 0.31}$  \\
7.50 & 50.73$^{+ 0.61}_{- 0.54}$  & 53.18$^{+ 0.16}_{- 0.46}$  \\
7.60 & 50.70$^{+ 0.52}_{- 0.66}$  & 52.79$^{+ 0.42}_{- 0.49}$  \\
7.70 & 51.16$^{+ 0.22}_{- 1.07}$  & 52.14$^{+ 0.35}_{- 0.65}$  \\
7.80 & 50.48$^{+ 0.58}_{- 0.87}$  & 52.76$^{+ 0.11}_{- 1.24}$  \\
7.90 & 51.06$^{+ 0.50}_{- 1.16}$  & 52.00$^{+ 0.59}_{- 1.18}$  \\
8.00 & 51.48$^{+ 0.26}_{- 1.77}$  & 51.55$^{+ 0.46}_{- 1.33}$  \\
\hline
\hline
% Element & \multicolumn{2}{c}{$A_X/A_{X\odot}$} \\
Element & F.I.P. (eV) &  $A_X/A_{X\odot}$ \\
\hline
C  & 11.26 &  0.73$^{+ 0.28}_{- 0.16}$ \\ 
N  & 14.53 &  0.85$^{+ 0.35}_{- 0.15}$ \\ 
O  & 13.62 &  0.54$^{+ 0.16}_{- 0.08}$ \\ 
Ne & 21.57 &  0.91$^{+ 0.30}_{- 0.16}$ \\ 
Mg &  7.65 &  0.41$^{+ 0.19}_{- 0.10}$ \\ 
Fe &  7.90 &  0.26$^{+ 0.07}_{- 0.05}$ \\ 
% C & \multicolumn{2}{c}{ 0.89$^{+ 0.12}_{- 0.34}$} \\ 
% N & \multicolumn{2}{c}{ 0.87$^{+ 0.15}_{- 0.24}$} \\ 
% O & \multicolumn{2}{c}{ 0.53$^{+ 0.06}_{- 0.10}$} \\ 
% Ne & \multicolumn{2}{c}{ 0.91$^{+ 0.08}_{- 0.21}$} \\ 
% Mg & \multicolumn{2}{c}{ 0.46$^{+ 0.09}_{- 0.15}$} \\ 
% Fe & \multicolumn{2}{c}{ 0.25$^{+ 0.03}_{- 0.06}$} \\ 
\hline\\
\end{tabular}
}
\end{center}
Abundances are in solar units (Anders \& Grevesse 1989, GeCoA, 53, 97).
\normalsize
\end{table}


